Does the Generator Mind its Contexts? An Analysis of Generative Model Faithfulness under Context Transfer

The present study introduces the knowledge-augmented generator, which is specifically designed to produce information that remains grounded in contextual knowledge, regardless of alterations in the context. Previous research has predominantly focused on examining hallucinations stemming from static input, such as in the domains of summarization or machine translation. However, our investigation delves into the faithfulness of generative question answering in the presence of dynamic knowledge. Our objective is to explore the existence of hallucinations arising from parametric memory when contextual knowledge undergoes changes, while also analyzing the underlying causes for their occurrence. In order to efficiently address this issue, we propose a straightforward yet effective measure for detecting such hallucinations. Intriguingly, our investigation uncovers that all models exhibit a tendency to generate previous answers as hallucinations. To gain deeper insights into the underlying causes of this phenomenon, we conduct a series of experiments that verify the critical role played by context in hallucination, both during training and testing, from various perspectives.

==> Body/Abstract.tex <==
\begin{abstract}
The knowledge-augmented generator is designed to generate information that is grounded in input contextual knowledge, regardless of how the context changes. Previous research has primarily focused on analyzing hallucinations from static input, such as in summarization or machine translation. However, in this study, we investigate the faithfulness of generative question answering with dynamic knowledge. We aim to explore whether hallucinations from parametric memory exist when contextual knowledge changes and analyze the reasons for their occurrence. For efficiency, we propose a simple and effective measure for detecting such hallucinations. Interestingly, our investigation reveals that all models hallucinate previous answers. To further understand the cause of this issue, we conduct experiments and verify that context plays a critical role in hallucination during both training and testing from several different perspectives. 
\end{abstract}

==> Table/Debatepedia/context_aug_results.tex <==
\begin{table}
  \centering
  \small
%   \scriptsize
  \begin{tabular}{lcc}
    \toprule
    \multirow{2}{*}{\bfseries Model} & \multicolumn{2}{c}{\bfseries Decoding Strategy} \\
    \cmidrule(r){2-3} 
       & {\bfseries Greedy} & {\bfseries Beam Search}  \\
    \hline

    T5$_{base}$              & 5.52$_{\downarrow 2.01}$ & 5.35$_{\downarrow 0.84}$ \\
    BART$_{large-xsum}$      & 5.35$_{\downarrow 2.68}$ & 7.02$_{\downarrow 0.17}$ \\
    \hline
    FiD (T5$_{base}$)        & 10.70$_{\downarrow 0.34}$ & 8.86$_{\downarrow 1.17}$ \\
    FiD (BART$_{large-xsum}$)& 13.55$_{\downarrow 2.03}$ & 11.54$_{\downarrow 3.01}$ \\
    
    
    \bottomrule
  \end{tabular}
  
  \caption{The $\mathcal{MFR}$(BERT-Score) results from augmented contexts. We generate text by greedy and beam search (beam=4) decoding strategy.}
  \label{Tab:Context_Aug}
\end{table}
